Flavour Physics and CP Violation

These lectures provide a concise introduction to flavor physics, within and beyond the Standard Model, with main focus on B-physics phenomenology and some recent developments. The first lecture is an introduction to the flavor sector of the Standard Model. The second lecture is devoted to B-meson mixing and rare B decays. The last lecture contains a general discussion about flavor physics beyond the Standard Model, with a highlighting of recent developments related to the idea of flavor deconstruction.

==> Mycommands.tex <==
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{dsfont}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{calc}
\usepackage{cancel}
\usepackage{slashed}
\usepackage{mathrsfs}
\usepackage{pdfpages}
\usepackage{tabu}
\usepackage{simplewick}
\usepackage{braket}
\usepackage{cite}
\usepackage{booktabs}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{array}}
\newcommand{\eeqa}{\end{array}}
\newcommand{\bim}{\begin{itemize}}
\newcommand{\eim}{\end{itemize}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\epoe}{\epsilon'/\epsilon}
\newcommand{\cA}{{\cal A}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cB}{{\cal B}}
\newcommand{\BR}{{\cal B}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cC}{C}
\newcommand{\SU}{{\rm SU}}
\newcommand{\UU}{{\rm U}}
\newcommand{\heavy}{{[3]}}
\newcommand{\light}{{[12]}}
\newcommand{\bsll}{b\to s\hspace{0.3mm}\ell^+\ell^-}
\newcommand{\dis}{\displaystyle}
\newcommand{\no}{\nonumber}
\newcommand{\yuk}{{\lambda}}
\newcommand{\Btaun}{{B \to \tau \nu}}
\newcommand{\kpn}{K^+\to\pi^+\nu\bar\nu}
\newcommand{\klpn}{K_L\to\pi^0\nu\bar\nu}
\newcommand{\kno}{{K^0}}
\newcommand{\knb}{{\overline{K}^0}}
\newcommand{\Gno}{\Gamma_{K^0}}
\newcommand{\Gnb}{\Gamma_{\overline K^0}}
\newcommand{\sla}{\! \! \! \!  /~}
\newcommand{\rhob}{\bar\varrho}
\newcommand{\etab}{\bar\eta}
\newcommand{\lsim}{\stackrel{<}{_\sim}}
\newcommand{\gsim}{\stackrel{>}{_\sim}}
\newcommand{\vev}[1]{\langle #1 \rangle}
\newcommand{\Tr}{\mbox{\rm Tr}}
\renewcommand{\Im}{{\rm Im}\,}
\renewcommand{\Re}{{\rm Re}\,}
\newcommand{\ssb}{\quad\Rightarrow\quad}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


